Leveraging Vision-Language Models for Improving Domain Generalization in Image Classification

Vision-Language Models (VLMs) such as CLIP are trained on large amounts of image-text pairs, resulting in remarkable generalization across several data distributions. However, in several cases, their expensive training and data collection/curation costs do not justify the end application. This motivates a vendor-client paradigm, where a vendor trains a large-scale VLM and grants only input-output access to clients on a pay-per-query basis in a black-box setting. The client aims to minimize inference cost by distilling the VLM to a student model using the limited available task-specific data, and further deploying this student model in the downstream application. While naive distillation largely improves the In-Domain (ID) accuracy of the student, it fails to transfer the superior out-of-distribution (OOD) generalization of the VLM teacher using the limited available labeled images. To mitigate this, we propose Vision-Language to Vision - Align, Distill, Predict (VL2V-ADiP), which first aligns the vision and language modalities of the teacher model with the vision modality of a pre-trained student model, and further distills the aligned VLM representations to the student. This maximally retains the pre-trained features of the student, while also incorporating the rich representations of the VLM image encoder and the superior generalization of the text embeddings. The proposed approach achieves state-of-the-art results on the standard Domain Generalization benchmarks in a black-box teacher setting as well as a white-box setting where the weights of the VLM are accessible.

==> suppl_tables/distill_ext_comp.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Distillation to lower capacity student models (extended comparisons):} Performance (\%) of the proposed approach VL2V-ADiP (denoted as
Ours), when compared to the KD and ERM finetune baselines with SWAD (S), with different student architectures. The teacher architecture is ViT-B/16 in all cases.}
\label{tab:distill_ext_comp}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}

\toprule
\textbf{Student} & \textbf{Method} & \textbf{OH} & \textbf{TI} & \textbf{VLCS} & \textbf{PACS} & \textbf{DN} & \textbf{Avg. (OOD)} \\ \midrule


\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ViT-B/16\\ (86M)\end{tabular}} & ERM (S) & 83.22 & 50.05 & 80.33 & 90.28 & 56.10 & 72.00 \\
 & KD (S) & 82.73 & 48.40 & 80.48 & 91.46 & 56.17 & 71.85 \\
 & Ours & \textbf{85.74} & \textbf{55.43} & \textbf{81.90} & \textbf{94.94} & \textbf{59.38} & \textbf{75.48} \\ \midrule

 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ViT-S/16\\ (22M)\end{tabular}} & ERM (S) & 78.58 & 49.40 & 78.72 & 85.80 & 52.09 & 68.92 \\
 & KD (S) & 78.14 & 50.11 & 79.14 & 85.97 & 52.05 & 69.08 \\
 & Ours & \textbf{81.22} & \textbf{52.47} & \textbf{81.44} & \textbf{89.32} & \textbf{54.23} & \textbf{71.73} \\ \midrule

 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}DeiT-S/16\\ (22M)\end{tabular}} & ERM (S) & 74.95 & 47.85 & 79.37 & \textbf{89.22} & 49.18 & 68.12 \\
 & KD (S) & 74.65 & 48.11 & 78.86 & 88.14 & 49.10 & 67.77 \\
 & Ours & \textbf{77.63} & \textbf{48.72} & \textbf{81.89} & 88.97 & \textbf{50.37} & \textbf{69.52} \\ \midrule

 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ResNet-50\\ (26M)\end{tabular}} & ERM (S) & 70.85 & 49.47 & \textbf{79.50} & \textbf{88.05} & 46.43 & 66.86 \\
 & KD (S) & 70.67 & 51.22 & 78.63 & 87.23 & 46.31 & 66.81 \\
 & Ours & \textbf{74.42} & \textbf{53.46} & 79.23 & 86.72 & \textbf{47.74} & \textbf{68.31} \\ \bottomrule
\end{tabular}%
}
\end{table}

==> suppl_tables/dom_split_dn_ad.tex <==
\label{tab:ad_dom_split}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}

\toprule
\multicolumn{1}{c}{\textbf{Method}} & \textbf{Clipart} & \textbf{Infograph} & \textbf{Painting} & \textbf{Quickdraw} & \textbf{Real} & \textbf{Sketch} & \textbf{Avg.} \\ \midrule
ERM-LP & & & & & & &\\
ERM Full Fine-Tuning & 76.34 & 30.92 & 64.76 & 21.30 & 77.70 & 65.60 & 56.10 \\
LP-FT \cite{LP-FT} & & & & & & & \\
SimKD \cite{SimKD} & & & & & & & \\
KD \cite{hinton2015distilling} & 76.56 & 31.29 & 64.55 & \textbf{21.44} & 77.62 & 65.23 & 56.11 \\
MIRO \cite{MIRO} & 76.32 & 30.96 & 64.52 & 20.18 & 77.88 & 64.63 & 55.75 \\
DART \cite{DART} & 77.62	& 34.14	& 67.64	& 21.05	& 80.73	& 67.11	& 58.05 \\
SAGM \cite{SAGM} & 76.67	& 29.85	& 64.42	& 20.68	& 77.58	& 64.58	& 55.63 \\
Text2Concept \cite{SAGM} & & & & & & & \\
RISE \cite{RISE} & & & & & & & \\
\textbf{VL2V-ADiP (Ours)} & \textbf{78.80} & \textbf{36.86} & \textbf{69.21} & 21.32 & \textbf{81.33} & \textbf{68.79} & \textbf{59.38} \\ \bottomrule
\end{tabular}%
}

==> suppl_tables/dom_split_dn_sd.tex <==
\label{tab:sd_dom_split}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccccc@{}}

\toprule
\multicolumn{1}{c}{\textbf{Method}} & \textbf{Clipart} & \textbf{Infograph} & \textbf{Painting} & \textbf{Quickdraw} & \textbf{Real} & \textbf{Sketch} & \textbf{Avg.} \\ \midrule

Zero-Shot \cite{CLIP} & 72.61 & 47.08 & 66.02 & 14.13 & \textbf{83.12} & 63.18 & 57.69 \\
ERM Full Fine-Tuning & 77.10 & 38.32 & 66.13 & \textbf{25.02} & 75.19 & 65.76 & 57.92 \\
MIRO \cite{MIRO} & 79.70 & 43.50 & 67.36 & 24.62 & 79.22 & 68.42 & 60.47 \\
DART \cite{DART} & 78.51	& 39.99	& 66.89	& 25.85	& 76.37	& 68.29	& 59.32 \\
SAGM \cite{SAGM} & 78.78	& 40.21	& 67.31	& 24.18	& 76.29	& 67.54	& 59.05 \\
LP-FT \cite{LP-FT} & & & & & \\
FLYP \cite{FLYP} & & & & & \\
CLIPood \cite{CLIPood} & & & & & \\
WiSE-FT \cite{WISE-FT} & & & & & \\
RISE \cite{RISE} & & & & & \\
\textbf{VL2V-SD (Ours)} & \textbf{79.96} & \textbf{49.00} & \textbf{71.05} & 23.34 & 82.05 & \textbf{71.36} & \textbf{62.79} \\ \bottomrule

\end{tabular}%
}

==> suppl_tables/dom_split_pacs_ad.tex <==
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\multicolumn{1}{c}{\textbf{Method}} & \textbf{Art} & \textbf{Cartoon} & \textbf{Photo} & \textbf{Sketch} & \textbf{Avg.} \\ \midrule

ERM-LP & & & & & \\
ERM Full Fine-Tuning & 93.78 & 86.25 & 99.18 & 81.93 & 90.28 \\
LP-FT \cite{LP-FT} & & & & & \\
SimKD \cite{SimKD} & & & & & \\
KD \cite{hinton2015distilling} & 94.20 & 86.35 & 99.25 & 86.04 & 91.46 \\
MIRO \cite{MIRO} & 94.69 & 85.98 & 99.63 & 77.70 & 89.50 \\
DART \cite{DART} & 94.45	& 86.67	& 99.55	& 81.52	& 90.55 \\
SAGM \cite{SAGM} & 93.72	& 86.57	& 99.18	& 80.63	& 90.02 \\
Text2Concept \cite{text2concept} & & & & & \\
RISE \cite{RISE} & & & & & \\
\textbf{VL2V-ADiP (Ours)} & \textbf{95.61} & \textbf{92.38} & \textbf{99.85} & \textbf{88.68} & \textbf{94.13} \\ \bottomrule
\end{tabular}%
}

==> suppl_tables/dom_split_pacs_sd.tex <==
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccc}

\toprule
\multicolumn{1}{c}{\textbf{Method}} & \textbf{Art} & \textbf{Cartoon} & \textbf{Photo} & \textbf{Sketch} & \textbf{Avg.} \\ \midrule

Zero-Shot \cite{CLIP} & 97.44 & \textbf{99.31} & \textbf{99.93} & 89.44 & 96.53 \\
ERM Full Fine-Tuning & 91.34 & 89.07 & 97.53 & 87.47 & 91.35 \\
MIRO \cite{MIRO} & \textbf{98.05} & 97.50 & 99.78 & 90.46 & 96.44 \\
DART \cite{DART} & 94.45 & 92.27 & 98.80 & 88.20 & 93.43 \\
SAGM \cite{SAGM} & 95.18	& 93.60	& 99.03	& 89.41	& 94.30 \\
LP-FT \cite{LP-FT} & & & & & \\
FLYP \cite{FLYP} & & & & & \\
CLIPood \cite{CLIPood} & & & & & \\
WiSE-FT \cite{WISE-FT} & & & & & \\
RISE \cite{RISE} & & & & & \\
\textbf{VL2V-SD (Ours)} & \textbf{98.05} & 98.19 & \textbf{99.93} & \textbf{90.55} & \textbf{96.68} \\
\bottomrule
\end{tabular}%
}

==> suppl_tables/dom_split_ti_ad.tex <==
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\multicolumn{1}{c}{\textbf{Method}} & \textbf{L100} & \textbf{L38} & \textbf{L43} & \textbf{L46} & \textbf{Avg.} \\ \midrule

ERM-LP & & & & & \\
ERM Full Fine-Tuning & 58.98 & 37.76 & 58.31 & 45.15 & 50.05 \\
LP-FT \cite{LP-FT} & & & & & \\
SimKD \cite{SimKD} & & & & & \\
KD \cite{hinton2015distilling} & 61.09 & 33.21 & 57.84 & 41.17 & 48.33 \\
MIRO \cite{MIRO} & 61.27 & 38.14 & 57.68 & 44.08 & 50.30 \\
DART \cite{DART} & 56.82	& 37.34	& \textbf{62.31} & 42.26 & 49.68 \\
SAGM \cite{SAGM} & \textbf{64.17} & 44.42 & 59.64 & 44.74 & 53.24 \\
Text2Concept \cite{text2concept} & & & & & \\
RISE \cite{RISE} & & & & & \\
\textbf{VL2V-ADiP (Ours)} & 62.93 & \textbf{44.83} & 60.71 & \textbf{53.26} & \textbf{55.43} \\
\bottomrule
\end{tabular}%
}

==> suppl_tables/dom_split_ti_sd.tex <==
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\multicolumn{1}{c}{\textbf{Method}} & \textbf{L100} & \textbf{L38} & \textbf{L43} & \textbf{L46} & \textbf{Avg.} \\ \midrule

Zero-Shot \cite{CLIP} & 51.65 & 20.03 & 33.60 & 31.49 & 34.19 \\
ERM Full Fine-Tuning & 38.94 & 38.03 & 54.03 & 40.68 & 42.92 \\
MIRO \cite{MIRO} & 67.15 & \textbf{50.75} & \textbf{66.63} & 52.71 & \textbf{59.31} \\
DART \cite{DART} & 56.82	& 37.34	& 62.31	& 42.26	& 49.68 \\
SAGM \cite{SAGM} & 72.21	& 50.10	& 62.50	& 49.73	& 58.64 \\
LP-FT \cite{LP-FT} & & & & & \\
FLYP \cite{FLYP} & & & & & \\
CLIPood \cite{CLIPood} & & & & & \\
WiSE-FT \cite{WISE-FT} & & & & & \\
RISE \cite{RISE} & & & & & \\
\textbf{VL2V-SD (Ours)} & \textbf{69.10} & 48.40 & 63.10 & \textbf{53.56} & 58.54 \\
\bottomrule
\end{tabular}%
}

==> suppl_tables/dom_split_vlcs_ad.tex <==
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccc}

\toprule
\multicolumn{1}{c}{\textbf{Method}} & \textbf{Caltech} & \textbf{LabelMe} & \textbf{VOC07} & \textbf{SUN09} & \textbf{Avg.} \\ \midrule

ERM-LP & & & & & \\
ERM Full Fine-Tuning & 98.49 & 64.05 & 82.60 & 76.17 & 80.33 \\
LP-FT \cite{LP-FT} & & & & & \\
SimKD \cite{SimKD} & & & & & \\
KD \cite{hinton2015distilling} & 98.87 & 65.32 & 81.33 & 76.39 & 80.48 \\
MIRO \cite{MIRO} & \textbf{99.75} & 64.79 & 82.66 & 77.20 & 81.10 \\
DART \cite{DART} & 94.08	& 63.11	& 76.12	& 75.86	& 77.29 \\
SAGM \cite{SAGM} & 98.49	& 64.92	& 79.32	& 75.68	& 79.60 \\
Text2Concept \cite{text2concept} & & & & & \\
RISE \cite{RISE} & & & & & \\
\textbf{VL2V-ADiP (Ours)} & 99.62 & \textbf{66.60} & \textbf{82.87} & \textbf{78.46} & \textbf{81.89} \\ \bottomrule
\end{tabular}%
}

==> suppl_tables/dom_split_vlcs_sd.tex <==
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccc}

\toprule
\multicolumn{1}{c}{\textbf{Method}} & \textbf{Caltech} & \textbf{LabelMe} & \textbf{VOC07} & \textbf{SUN09} & \textbf{Avg.} \\ \midrule

Zero-Shot & \textbf{100.00} & \textbf{69.02} & 84.19 & 74.86 & 82.02 \\
ERM Full Fine-Tuning & 99.12 & 63.31 & 79.01 & 75.08 & 79.13 \\
MIRO \cite{MIRO} & 97.53 & 66.59 & 81.57 & \textbf{83.53} & 82.30 \\
DART \cite{SWAD} & 99.12 & 65.73 & 81.07 & 75.63 & 80.38 \\
SAGM \cite{SAGM} & 97.73 & 65.86 & 83.77 & 80.85 & 82.05 \\
LP-FT \cite{LP-FT} & & & & & \\
FLYP \cite{FLYP} & & & & & \\
CLIPood \cite{CLIPood} & & & & & \\
WiSE-FT \cite{WISE-FT} & & & & & \\
RISE \cite{RISE} & & & & & \\
\textbf{VL2V-SD (Ours)} & 99.24 & 67.81 & \textbf{86.89} & 79.05 & \textbf{83.25} \\
\bottomrule
\end{tabular}%
}
